Network Newton

We consider minimization of a sum of convex objective functions where the components of the objective are available at different nodes of a network and nodes are allowed to only communicate with their neighbors. The use of distributed subgradient or gradient methods is widespread but they often suffer from slow convergence since they rely on first order information, which leads to a large number of local communications between nodes in the network. In this paper we propose the Network Newton (NN) method as a distributed algorithm that incorporates second order information via distributed evaluation of approximations to Newton steps. We also introduce adaptive (A)NN in order to establish exact convergence. Numerical analyses show significant improvement in both convergence time and number of communications for NN relative to existing (first order) alternatives.

==> Implementation.tex <==
%!TEX root = root.tex

\section{Implementation issues} \label{sec:implement}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{algorithm}[t]{
\caption{Computation of NN-$K$ step at node $i$.}
\label{algo_NNK} 
\begin{algorithmic}[1]
   \STATE \textbf{function}  
          [$\|\bbg_{i,t}\|$, $\bbx_{i,t+1}$]
          = NN-$K$ Step$\left(\alpha_t, \bbx_{i,t} \right)$ 
   %%% First for loop   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \STATE $\bbB$ matrix blocks: $\bbB_{ii}=(1-w_{ii})\bbI$ and $\bbB_{ij}=w_{ij}\bbI$
   \STATE $\bbD$ matrix block: $\bbD_{ii,t}= \alpha_t \nabla^2 f_{i}(\bbx_{i,t}) + 2(1-w_{ii})\bbI $
   \STATE Exchange iterates $\bbx_{i,t}$ with neighbors $j\in \mathcal{N}_i$.
   \STATE Gradient:    
          %
          $\displaystyle{
          \bbg_{i,t} = (1-w_{ii})\bbx_{i,t} 
                       - \sum_{j\in \mathcal{N}_i} w_{ij} \bbx_{j,t}
                       +\alpha_t \nabla f_{i}(\bbx_{i,t}).}$  
          %
   \STATE Compute NN-0 descent direction $\bbd_{i,t}^{(0)}=-\bbD_{ii,t}^{-1}\bbg_{i,t}$\\ 
   \FOR  {$k=  0, \ldots, K-1$ } 
      \STATE Exchange elements $\bbd_{i,t}^{(k)}$ of the NN-$k$ step with neighbors
      \STATE NN-$(k+1)$ step:
             %
             $\displaystyle{  
             \bbd_{i,t}^{(k+1)} = \bbD_{ii,t}^{-1}
             			\bigg[
                                   \sum_{j\in \mathcal{N}_i,j=i}\bbB_{ij} \bbd_{j,t}^{(k)} 
                                    - \bbg_{i,t}\bigg]}$.        
   \ENDFOR
  %  $\bbD_t_{N}(t)=$ NN Descent Direction $\left(\bbD_t_{0}(t), \bbg(t), N \right)$.
          %
          \STATE Update local iterate: 
          $\displaystyle{\bbx_{i,t+1}=\bbx_{i,t} +\eps\ \bbd_{i,t}^{(K)}}$.
    \STATE \{return $\|\bbg_{i,t}\|$ and $\bbx_{i,t+1}$\} 
\end{algorithmic}}\end{algorithm}



As mentioned in Section \ref{sec:problem}, NN-$K$ algorithm instead of solving  \eqref{original_optimization_problem1} or its equivalent  \eqref{original_optimization_new_notation}, solves a penalty version of \eqref{original_optimization_new_notation} as introduced in \eqref{centralized_opt_problem}. 
The optimal solutions of optimization problems \eqref{original_optimization_new_notation} and \eqref{centralized_opt_problem} are different and the gap between them is upper bounded by $O(\alpha)$ \cite{YuanQing}. This observation implies that by setting a decreasing policy for $\alpha$ or equivalently an increasing policy for penalty coefficient $1/\alpha$, the solution of  \eqref{original_optimization_new_notation} approaches the minimizer of  \eqref{centralized_opt_problem}, i.e. $\tby^* \to \bby^*$ for $\alpha\to  0$.

 
We introduce Adaptive Network Newton-$K$ (ANN-$K$) as a version of NN-$K$ that uses a decreasing sequence of $\alpha_t$ to achieve exact convergence to the optimal solution of \eqref{original_optimization_problem1}. The idea of ANN-$K$ is to decrease parameter $\alpha_t$ by multiplying by $\eta<1$, i.e., $\alpha_{t+1}=\eta\alpha_t$, when the sequence generated by NN-$K$ is converged for a specific value of $\alpha$. To be more precise, each node $i$ has a \textit{signal vector} $\bbs_{i}=[s_{i1};\dots;s_{in}]\in \{0,1\}^n$ where each component is a binary variable. Note that $s_{ij}$ corresponds to the occurrence receiving a signal at node $i$ from node $j$. Hence, nodes initialize their signaling components by $0$ for all the nodes in the network. At iteration $t$ node $i$ computes its local gradient norm $\|\bbg_{i,t}\|$. If the norm of gradient is smaller than a specific value called $tol$, i.e. $\|\bbg_{i,t}\|\leq tol$, it sets the local signal component to $s_{ii}=1$ and sends a signal to all the nodes in the network. The receiver nodes set the corresponding component of node $i$ in their local signal vectors to 1, i.e. $s_{ji}=1$ for $j\neq i$. This procedure implies that the signal vectors of all nodes in the network are always synchronous. The update for parameter $\alpha_t$ occurs when all the components of signal vector are 1 which is equivalent to achieving the required accuracy for all nodes in the network. Since the number of times that $\alpha_t$ should be updated is small, the cost of communication for updating $\alpha_t$ is affordable. 


The ANN-$K$ method is summarized in Algorithm \ref{algo_ANN}. At each iteration of ANN-$K$ algorithm at Step 2 function NN-$K$ Step is called to update variable $\bbx{i,t}$ for node $i$ and also return the norm of local gradient $\|\bbg_{i,t}\|$. Note that function NN-$K$ Step is introduced in Algorithm \ref{algo_NNK} and it is exactly similar to the step of NN-$K$ algorithm. The main differences of NN-$K$ and ANN-$K$ are in using time varying penalty parameter $\alpha_t$ and signal vectors $\bbs_i$ for updating penalty parameter. In Steps 3-6 node $i$ updates its local signal component $s_{ii}$ to $1$ and sends it to the other nodes if the accuracy $\|\bbg_{i,t}\|\leq tol$ is achieved. In Step 7 each node $i$ updates the signal vector components of other nodes in the network. Then, in Steps 8-13 the nodes update the penalty parameter for the next iteration as $\alpha_{t+1}=\eta\alpha_t $  if all the components of signal vector is 1, otherwise they use the previous value $\alpha_{t+1}=\alpha_{t}$. In order to reset the system after updating $\alpha_t$, all local signal vectors set to 0, i.e. $\bbs_{i}=\bb0$ for $i=1,\dots,n$ as in Step 12.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M   %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{algorithm}[t]
\caption{Adaptive Network Newton-$K$ method at node $i$}\label{algo_ANN} 
\begin{algorithmic}[1] {
\REQUIRE  Initial iterate $\bbx_{i,0}$, initial penalty parameter $\alpha_0$ and initial sequence of bits $\bbs_i=[s_{i1};\dots;s_{in}]=[0;\dots;0].$
\FOR {$t=0,1,2,\ldots$}
     \STATE \textbf{function}  
          [$\|\bbg_{i,t}\|$, $\bbx_{i,t+1}$]
          = NN-$K$ Step$\left(\alpha_t, \bbx_{i,t} \right)$ 
   \IF{$\|\bbg_{i,t}\|\leq tol$}
   \STATE Set $s_{ii}=1$.
   \STATE Send scalar $1$ to all nodes.
   \ENDIF
   
   
   \STATE Set $s_{ij}=1$ for all nodes $j$ that sent a signal.

   
   \IF{$s_{ij}=1$ for all $j=1,\dots,n$}
   \STATE Update penalty parameter $\alpha_{t+1}=\eta\alpha_t.$
   \STATE Set $s_{ij}=0$ for all $j=1,\dots,n$.
   \ELSE
   \STATE Use the old $\alpha$: $\alpha_{t+1}=\alpha_t.$
   \ENDIF
   

\ENDFOR}
\end{algorithmic}\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   R   E   M   A   R   K   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{remark} \normalfont
One may think for achieving more exact convergence instead of using the ANN-$K$ method with decreasing $\alpha $ the NN-$K$ algorithm with very small penalty factor can be used, however, choosing very small $\alpha$ leads to very slow convergence for NN-$K$. By setting large $\alpha $ we try to minimize objective function $\sum_{i=1}^n f_{i}(\bbx)$ with less concern about the constraint $(\bbI-\bbZ)^{1/2}\bby=\bb0$. This leads to a point closer to the optimal solution. Then, by decreasing $\alpha $ we put more weight on the constraint and less on the objective function, while we use a better initial point than just starting the whole procedure with small $\alpha$. This is well studied in Section \ref{sec:simulations}.
\end{remark}






